Online Learning and Unlearning

We formalize the problem of online learning-unlearning, where a model is updated sequentially in an online setting while accommodating unlearning requests between updates. After a data point is unlearned, all subsequent outputs must be statistically indistinguishable from those of a model trained without that point. We present two online learner-unlearner (OLU) algorithms, both built upon online gradient descent (OGD). The first, passive OLU, leverages OGD's contractive property and injects noise when unlearning occurs, incurring no additional computation. The second, active OLU, uses an offline unlearning algorithm that shifts the model toward a solution excluding the deleted data. Under standard convexity and smoothness assumptions, both methods achieve regret bounds comparable to those of standard OGD, demonstrating that one can maintain competitive regret bounds while providing unlearning guarantees.

==> main_files/4-active.tex <==
The previous section~(\Cref{sec:passive}) passively exploits OGD’s properties but does not actively adjust the current output toward the retrained outputs. However, analyzing deterministic online gradient descent directly is complex, and to our knowledge, no existing work has done so. To address this, we introduce a framework in~\Cref{sec:general-active-unlearner} that leverages existing offline unlearning methods. While these methods are designed for an auxiliary offline learning algorithm rather than OGD, they can sometimes bring our algorithm’s output closer to the retrained output from a dataset without the deleted points, reducing the required noise and improving regret bounds.

In \Cref{sec:ERM}, we instantiate this framework with two existing unlearning algorithms, \citet{neel2020descenttodeletegradientbasedmethodsmachine} and \citet{Sekhari21Remember}, and compare their performance with our passive unlearning approach.


\subsection{General active unlearner}\label{sec:general-active-unlearner}
To develop an online unlearning approach, we consider an auxiliary (offline) learning algorithm, denoted by $\aux$, for which unlearning in the offline setting is well understood. We define the deterministic part of the unlearning algorithm (i.e., the steps performed before adding noise) for $\aux$ as $\Unaux$.  

We introduce the general active online learning and unlearning algorithm, denoted by $\cR_{\Unaux}$, which combines OGD as the base learner with $\Unaux$ as the deterministic unlearning procedure $\UnDet$ and an appropriate perturbator (see~\Cref{alg:general-active}). When there is no unlearning request, the algorithm follows OGD updates. When a deletion request occurs at time \( t_i \in \cT \), we first apply $\Unaux$ to unlearn the corresponding data point, then add Gaussian noise \( \eta_i \sim \cN(0, \sigma_i^2) \). 

Specifically, let $L_R$ denote the Lipschitzness of the deterministic unlearning procedure $\UnDet$ with respect to its first input $z\in \cK$, the amount of noise added at time $t_i$ is defined as \[\sigma_i= \sqrt{\frac{\alpha j^\omega \omega}{2(\omega -1)\varepsilon}}\br{\max_{z\in \cK}\norm{\Unaux(z, \trainsetsub{t_j}, \unlearnsetsub{j}) - \Unaux(z, \trainsetsub{t_j}\setminus \unlearnsetsub{j},\emptyset )}_2 + L_R \gamma^{t_i - u_i}\eta_{u_i}L},\]
where the first term measures the distortion due to the unlearning algorithm. 

The passive unlearning fits in this framework, by having 
\[\max_{z\in \cK}\norm{\Unaux(z, \trainsetsub{t_j}, \unlearnsetsub{j}) - \Unaux(z, \trainsetsub{t_j}\setminus \unlearnsetsub{j},\emptyset )}_2 = 0, \quad L_R = 1\]
Therefore, potentially, an active unlearning algorithm can allows for adding less noise, if the distortion of the unlearning algorithm is small and $L_R\leq 1$. 

The key idea is to use an unlearning algorithm designed for \(\aux\) to unlearn the active learner and unlearner, assuming that \(\aux\) behaves similarly to our online learner and unlearner. To establish a regret guarantee for the active unlearning algorithm, we define \( e_1 \) as the unlearning accuracy of the deterministic unlearning algorithm \(\Unaux\) relative to the offline auxiliary algorithm \(\aux\), \( e_3 \) as the stability of \(\aux\), and \( e_2 \) as the deviation between the outputs of our online learner and unlearner and those of \(\aux\). For \( S \in \cF^t \), 

\begin{equation}
    \label{eq:defn-e1-e2}
    \begin{aligned}
        e_1(t) &= \sup_{\trainset\subset \cF^t,\unlearnset\in \cK}\norm{\Unaux(\aux(\trainset), \trainset,\unlearnset) - \aux(\trainset \setminus \unlearnset)}_2\\
        e_2(\mathbf{\eta}, S, \cT, \cU, t) &= \bs{\OnUnalg(\eta, S, \cT, \cU)}_t- \aux(S\setminus S_U)\\
        e_3(t) &= \max_{x\in \cF, S\in \cF^{t}}\norm{\aux(S) - \aux(S\setminus \{x\})}_2.\\
    \end{aligned}
\end{equation}
where $\cA_{\textrm{OGD}, \eta}$ represents OGD with learning rate $\eta$ (which can be constant or a time-varying vector).

In~\Cref{thm:active-guarantee-general}, we establish the unlearning and accuracy guarantees for~\Cref{alg:general-active}. The unlearning guarantee applies to any base learner that satisfies~\Cref{condition:contractive,condition:markov,condition:sensitivity}, while the regret guarantee is specific to OGD as the base learner.


\begin{restatable}{theorem}{ActiveGeneral}
    \label{thm:active-guarantee-general}
    Let $\aux$ and $\Unaux$ be an auxiliary offline learning algorithm and a deterministic unlearning procedure with corresponding terms $e_1, e_2, e_3$ defined as in~\Cref{eq:defn-e1-e2}. Assume the cost functions are convex and $L$-Lipschitz, $\Unaux$ is $L_R$ Lipschitz, and the index of the unlearning point $u_i$ satisfies $u_i\in (t_{i-1}, t_i)$ for all $i\in [k]$. Then,~\Cref{alg:general-active} is an $(\alpha, \varepsilon)$-online unlearner, and its expected regret is upper bounded by
    \[\mathrm{Regret}(\cA_{\mathrm{OGD}, \eta}) + \sum_{i = 1}^k \bE\bs{\norm{\delta_i}_2} \br{L +  \frac{D}{\eta_{t_i}}} + \frac{\bE\bs{\norm{\delta_i}^2}}{2\eta_{t_i}} + \frac{\sigma_i^2}{2\eta_{t_i}},\]
    where $\norm{\delta_i}_2 \leq (L_R + 1) e_2(\eta_t, \cT, \cU, t_i) + e_1(t_i) + e_3(t_i)$.  
\end{restatable}


For strongly convex loss functions, if the auxiliary unlearning algorithm has a contractive coefficient $L_R$ smaller than 1 and its distortion rate, along with the error terms $e_1(t)$ $e_3(t)$, and $\bE\bs{\max_{S, \cT, \cU} e_2(\mathbf{\eta}, S, \cT, \cU, t)}$ for some $\eta$, are of order $O(1/t)$, then active unlearning with this auxiliary algorithm achieves a regret guarantee of $O(\log T)$ regardless of the deletion sets. This outperforms the deletion-set-independent regret bound of passive unlearning. As shown in~\Cref{thm:passive-worst-case,thm:regret-passive-unlearner-strongly-convex}, the passive unlearning algorithm guarantees a regret bound of $O(\sqrt{T})$, independent of the deletion set, or a logarithmic regret that depends on the deletion set.


\subsection{Using ERM as an auxiliary offline algorithm}\label{sec:ERM} 


In this section, we instantiate the active general unlearner by considering ERM as the auxiliary offline learning algorithm $\aux$. 

Of the many unlearning algorithms designed for ERM, we adapt from the first-order method, proposed by~\citet{neel2020descenttodeletegradientbasedmethodsmachine} and the second-order method, proposed by~\citet{Sekhari21Remember} due to their computational efficiency and certified unlearning guarantee. For the first-order method, we define the auxiliary unlearning algorithm to take as input all previous cost functions. It performs \(\cI_1\) gradient descent steps using all these cost functions, followed by \(\cI_2\) gradient descent steps using all those excluding the deleted points. The second-order unlearning algorithm also takes \(\cI_1\) gradient descent steps using all cost functions, followed by one reverse Newton update using the deleted functions. See~\Cref{alg:ERM-first-order,alg:ERM-second-order} for details of online unlearner instantiated with these auxiliary unlearning algorithms. 

Compared with the offline auxiliary unlearning algorithm in~\citet{neel2020descenttodeletegradientbasedmethodsmachine,Sekhari21Remember},  our online adaptation requires an additional $\cI_1$ steps of gradient descent over all previous cost functions. This is because offline methods adjust the the ERM solution on all data points to the ERM solution of the retaining set. However, the original OGD outputs may be far from the ERM solution. These extra steps help move the OGD output closer to ERM, providing a reasonable starting point for the offline unlearning algorithm. This ensures the unlearning guarantee holds with less noise addition. 


Because the unlearning algorithm shifts the original algorithm away from OGD outputs and towards an ERM solution upon deletion requests, we require an additional assumption to establish the regret guarantee.  Specifically, the error terms $e_1, e_2, e_3$ must be small (e.g. $O(1/t)$). Here $e_2$ represents the difference between our online unlearner~(\Cref{alg:general-active}) and the ERM solution. To control this difference, we propose~\Cref{assump:assumption1}, which assumes a positive angle between the gradient directions of any two possible cost functions at any point. This ensures that OGD convergence to the ERM solution.

\begin{assumption}\label{assump:assumption1}
Let the set $\cF$ be a set of cost functions such that $\forall f_i, f_j\in \cF$ and $\forall w\in \cW$, the following holds, 
\[\br{\nabla f_j(w)}^\top \nabla f_i(w) \geq 0. \]
\end{assumption}

Under this assumption, our proposed first-order and second-order unlearning algorithm satisfies the following theoretical guarantees~(\Cref{thm:first-order-guarantee}). 

\begin{theorem}
    \label{thm:first-order-guarantee}
    Assume all loss functions are $L$-Lipschitz, $\mu$-strongly convex, $\beta$-smooth, $M$-Hessian Lipschitz and satisfy~\Cref{assump:assumption1}. Assume the index of the unlearning point $u_i \in (t_{i-1}, t_i)$ for all $i$, then the the regret of the first-order and second-order online learning and unlearning algorithms is upper bounded by  \[\bE\text{Regret}_T \leq O\br{\log T + \sqrt{t_1t_2...t_k}}
    .\]
    assuming $\log t_k \sqrt{t_{k-1} \log t_{k-1}}$
\end{theorem}

The complete proof can be found in~\Cref{app:ERM}. 


% \subsection{Second-order method}\label{sec:ERM-second-order}
% Second-order information of the loss function has also been exploited in batch setting to achieve certified unlearning while maintaining model accuracy~\citep{Dong24IDEA,Sekhari21Remember,Guo19Certified}. Similar to the previous section, we consider the base learning algorithm to be online gradient descent. When receiving the $j$th deletion request, the unlearner performs Newton's update with the retaining set between $t_{j}$ and $t_{j-1}$. Then, Gaussian noise $\xi\sim \cN(0, \sigma_j^2)$ is added. The standard deviation $\sigma_j$ is defined as \[\sigma_j = \frac{2ML^2 \br{1 + \log \Delta_{t_j}} + t_{j-1}D}{\mu^3\Delta_{t_j}} + \br{\frac{2\beta}{\mu^2} + \frac{L}{\mu}}\sqrt{\frac{2\br{1 + \log \Delta_{t_j}} + t_{j-1}D}{\Delta_{t_j}}}. \]

% We denote the above algorithm as $\cR_{\cA}^{(2)}$, described in~\Cref{alg:second-order-online-learner-unlearner}. Under~\Cref{assump:assumption1}, $\cR_{\cA}^{(2)}$ is an $(\alpha, \varepsilon)$-online learner unlearner. 


% \begin{theorem}
%     \label{thm:second-order-guarantee}
%     Assume all loss functions are $L$-Lipschitz, $\mu$-strongly convex, $\beta$-smooth, and satisfy~\Cref{assump:assumption1}. Assume the index of the unlearning points satisfies $u_i \in (t_{i-1}, t_i)$. Then we can upper bound the regret of the competing algorithm of $\cR_{\cA}^{(2)}$ that unlearns an arbitrary point at time $\cT$ by \[\bE\text{Regret}_T \leq O\br{\log T + }.\]
% \end{theorem}




==> main_files/6-extensions.tex <==



\subsection{User-level deletion}
\begin{assumption}\label{assump:user-level-unlearning}
    Each user $i$ contribute at most $m$ point until they make an unlearning request. 
\end{assumption}

We denote the set of deletion indices for user $i$ as $\cU_i = \{u^{(i)}_1, ..., u^{(i)}_m\}$, and denote deletion index set for all users as $\cU = \{\cU_i\}_{i = 1}^k$. Assume the user $i$ makes deletion request at time $t_i$, and denote the time set as $\cT$. 

Given $\cU$ and $\cT$,~\Cref{alg:unlearning-general} achieves user-level unlearning guarantee with parameters $\varepsilon, \delta$, when~\Cref{eq:general-unlearning-noise} is replaced by 
\begin{equation}\label{eq:general-unlearning-noise-userlevel}
    \zeta_t = \begin{cases}
    \mathcal{N}\br{0, \frac{\sum_{j = 1}^m\lambda^{2\br{t_i - u_j^{(i)}}}\Delta^2} {\varepsilon^2}}& \text{if } t_i \in T, \\
    0 & \text{otherwise.}
\end{cases}
\end{equation}

We can compute the expected regret of the user-level online learning unlearning algorithm by replacing the variance in~\Cref{eq:general-unlearning-noise} by~\Cref{eq:strong-convexity}, which we summarized as follows
\begin{itemize}
    \item \textbf{Strongly convex} \[\frac{L^2}{\gamma}(1+\log T) + \frac{\gamma k}{2\varepsilon}\sum_{i = 1}^k \sum_{j = 1}^m t_i\lambda^{2(t_i - u_j^{(i)})},\] where $\lambda = \frac{\beta/\gamma - 1}{\beta/\gamma + 1}$. 
    \item \textbf{Convex} \[6DL\sqrt{T} + \sum_{i = 1}^k \frac{mL}{2(t_i - 1)\varepsilon}. \]
\end{itemize}

One can restrict the number of contributions per user by stopping updates with the same user's data once their contributions exceed $m$ points. This ensures that the unlearning guarantee holds even if~\Cref{assump:user-level-unlearning} is not met. However, we note that this approach can introduce additional bias into the learning process and lead to a degradation in the expected regret.

Assume each user $i$ contributes $c_i$ data points, and let $E = \sum_{i} c_i - m$ denote the total number of points where no update is performed. Then the expected cumulative regret increase by $ED^2$ for both convex and strongly convex case. 
% \begin{restatable}[Regret for exp-concave loss]{thm}{RegretExpConcave}\label{thm:acc-exp-concave}
% For $\beta$-smooth loss and $\alpha$-exp concave loss function $\ell$, given a deletion index set $\cJ$ and a deletion time set $\cT$, the continual unlearning algorithm~\Cref{alg:learning-unlearning-online-newton} achieves the following guarantee for all $T\geq 1$, the expected regret is 
% \[O\br{\br{\frac{1}{\alpha} + LD} \br{d\log \br{\frac{T}{d}} + d\log \br{d+\frac{k\beta^2 (1+L)}{ \varepsilon^2}}}}.\]
% \end{restatable}

\subsection{Differential private online convex optimization}
Next, we compare our algorithms with unlearning with differentially private online convex optimization~\citep{Smith13OptimalPrivateOnlineLearning,Prateek12DPOnline}.

PGIGA\citep{Prateek12DPOnline}, Strong convex loss 
\[\frac{4\sqrt{kd}\br{\frac{L}{\mu} + D}L\log^2\frac{T}{\delta}}{\sqrt{\epsilon}}\sqrt{T} + \frac{2L^2\br{1 + \log T}}{\mu} + O(1)\]

For quadratic loss, DP-FTL\citep{Prateek12DPOnline}
\[\tilde{O}\br{\frac{D^6\sqrt{k}\log\frac{1}{\delta}}{\sqrt{\epsilon}\mu^3}}\sqrt{d}\log^{1.5}T\]

Lipschitz and strong convex loss, DP-FTAL~\citep{Smith13OptimalPrivateOnlineLearning}
\[O\br{\frac{kd\log^{2.5}T}{\varepsilon}}\]

==> main_files/online_unlearning.tex <==

Given learning algorithm $\cA$, then at time $t$, $\cA$ maps a set of history $(x_1, ..., x_{t-1})$ to a point $x_t^\cA = \cA(x_1, ..., x_{t-1})\in \cK$. We write $x_{t:T}^\cA$ as the output of the algorithm at time $t$ to $T$. Assume at time $t$, the algorithm $\cA$ predicts with $x^\cA_{t-1}$ and $(x_{t-1}, y_{t-1})$. 


Let $\cA$ be an online learning algorithm and let $\cO$ be an output space. For every time step $t$
\begin{itemize}
    \item Adversary chooses a point, $(x_t, y_t)$
    \item The online learning algorithm receives its output at the last time step $o_{t-1}$ and the point $x_t$, and predicts $\hat{y}_t$ based on $o_{t-1}$. 
    \item The online learning algorithm receives the correct output $y_t$, suffers from loss $\ell(y_t, \hat{y}_t)$ and update its output $o_t = \cA(o_{t-1}, (x_t, y_t))$. 
\end{itemize}

For a sequence of points $S_T = \{(x_t, y_t)\}_{t = 1}^T$, denote the output of an algorithm $\cA$ on $S_T$ as $O_\cA(S_T) = \{o_1, ..., o_T\}$, where $o_t = \cA(o_{t-1}, (x_t, y_t))$. 

\begin{defn}[Time-specific $(\alpha, \epsilon)$-online unlearning of a single point]
    For any $\alpha > 1$, an online unlearning algorithm $U$ is said to $(\alpha, \epsilon)$-online unlearn the $j^{\text{th}}$ point at time $t$ from an algorithm $\cA$ if there exists an online learning algorithm $\cA'$ such that for any sequence of data points $S = \{(x_i, y_i)\}_{i = 1}^t$,\[\rdp{U([O_\cA(S)]_t, x_j, \cI)}{[O_{\cA'}(S\setminus \{x_j\})]_{t-1}}\leq \epsilon,\]
    where $[O]_t$ denote the $t^{\text{th}}$ element of a vector $O$ and $\cI$ is a set of auxiliary information. 
\end{defn}

We note that the output $o_t$ can be considered as post-processing of $o_{t-1}$. By data processing inequality, if $\rdp{o_t}{\tilde{o}_t} \leq \alpha$, then $\rdp{o_{t'}}{\tilde{o}_{t'}}\leq \alpha$ for all $t'\geq t$. 

\begin{defn}[Time specific $(\alpha, \epsilon)$-online sequential unlearing]\label{defn:sequential-unlearning}
    For any $\alpha > 1$, an unlearning algorithm $U$ is said to $(\alpha, \epsilon)$-online unlearn a set of $k$ points $\cJ = \{j_1, ..., j_k\}$ at times $\cT = \{t_1, ..., t_k\}$ from an online learning algorithm $\cA$ if there exists a series of online learning algorithm $\cA_1, ..., \cA_k$ such that for any sequence of data points $S = \{(x_i, y_i)\}_{i = 1}^T$, for all $i \in [k-1]$, 
    \begin{equation}\label{eq:defn-unlearning-guarantee-sequential}
    \begin{aligned}
        &\rdp{U([O_{\cA_{i}}(S\setminus\{x_{j_1:j_i}\}]_{t_{i+1}}, x_{j_{i + 1}})}{O_{\cA_{i+1}}(S\setminus \{x_{j_1: j_{i+1}}\})]_{t_{i+1} - i-1}}\\&\leq\epsilon,
    \end{aligned}
    \end{equation}
    where $\cI$ is a set of auxiliary information. 
\end{defn}

